A stacky approach to prismatic crystals via $q$-prism charts

Let $Y$ be a locally complete intersection over $\mathcal{O}_K$ containing a $p$-power root of unity $\zeta_p$. We classify the derived category of prismatic crystals on the absolute prismatic site of $Y$ by studying quasi-coherent complexes on the prismatization of $Y$ via $q$-prism charts. We also develop a Galois descent mechanism to remove the assumption on $\mathcal{O}_K$. As an application, we classify quasi-coherent complexes on the Cartier-Witt stack and give a purely algebraic calculation of the cohomology of the structure sheaf on the absolute prismatic site of $\mathbb{Z}_p$. Along the way, for $Y$ a locally complete intersection over $\overline{A}$ with $A$ lying over a $q$-prism, we classify quasi-coherent complexes on the relative prismatization of $Y$.

==> trash.tex <==
%@article{cai24,
title="{Trivializing $\widehat{\mathcal{O}}_{\mathbb{G}_m^{\sharp}}$}-comodules explicitly",
  author={Hanlin Cai},
 howpublished ={\url{https://www.math.columbia.edu/~hanlin/Trivializing_Sen_Operator.pdf}},
}

\begin{remark}
    Our assumption really means that $(A,I)$ is an object in the prismatic site of the $\delta$-pair $(W(k)[[q-1]], \mathbb{Z}_p[\zeta_p])$ in the sense of \cite[Definition 2.4]{antieau2023prismatic} (but $I$ might not be generated by $[p]_q$). We prefer to work in this generality to emphasize the philosophy that prismatic crystals on the relative prismatic site are in fact independent of the prism structure and only depend on the underlying $\delta$-ring, advertised in \cite{antieau2023prismatic}.
\end{remark}
\begin{remark}\label{rem.appl. eta on the structure sheaf}
    Notice that $\mathfrak{S}\{\frac{p^m}{E}\}_{\delta}^{\wedge}$ is the $p$-adic completion of $\mathfrak{S}[\delta^{i}(T)_{i\geq 0}]/(\delta^{i}(Et-p^m)_{i\geq 0})$, under this explicit interpretation, one can show that $\eta(u)=E(u)$ and
    $$
        \eta(t)=t(1-\epsilon E^{\prime}(u)),\qquad \qquad~\eta(\delta^i(t))=\delta^i(t)+(-1)^{i-1}(\prod_{j=0}^{i-1}\delta^{j}(t))^{p-1}tE^{\prime}(u)\epsilon, ~~~i\geq 1.
    $$
\end{remark}

\begin{proposition}\label{prop. lci relative c to construct homotopy}
For any $x\in \XY$, there exists a unique $c_{\psi}(x)$ in $W(\XY\otimes_{\Tilde{R}} S)$ such that $$\Tilde{\psi}_(x)-\Tilde{\iota}(x)=d \cdot c_{\psi}(x).$$
Here $\Tilde{\psi}$ is the unique $\delta$-ring morphism such that the following diagram commutes:
    \[\begin{tikzcd}[cramped, sep=large]
& W(\XY\otimes_{\Tilde{R}} S) \arrow[d, "p_0"]\\ 
\XY \arrow[ru, "\Tilde{\psi}"] \arrow[r, "\psi"]& \XY\otimes_{\Tilde{R}} S
\end{tikzcd}\]
and $\Tilde{\iota}$ is defined similarly with the bottom line in the above diagram replaced with the natural inclusion $\iota: \Tilde{R}\hookrightarrow S$. 
\end{proposition}
\begin{proof}
    
\end{proof}


\begin{remark}\label{rem. relative category}
    $\gamma_{c_{\psi_{}}}$ gives a $\psi$-linear endomorphism on $\rho^{*}(\mathscr{E})\otimes_{\Tilde{R}} S \in \mathcal{D}(S)$, hence $(\rho^{*}(\mathscr{E}),\gamma_{c_{\psi_{}}})$ lies in the category $\mathcal{C}_1$ defined to be the pullback of the following square:
    \[ \xymatrix{ \mathcal{C}_1 \ar[d] \ar[r] &   \mathcal{D}(\Tilde{R}) \ar[d] \\ 
\operatorname{Fun}(\Delta^{1}, \mathcal{D}(S)) \ar[r] & \operatorname{Fun}(\Delta^{0}\sqcup \Delta^{0}, \mathcal{D}(S)) }.\]
Here the arrow in the bottom is the forgetful functor sending $(M\xrightarrow[]{f} N)$ to $(M,N)$ for $M, N\in \mathcal{D}(S)$ and the right vertical map sends $K \in  \mathcal{D}(\Tilde{R})$ to $(\psi^{*}K, K\otimes_{\Tilde{R}} S)$.

Similarly, one could define the category $\mathcal{C}_2$ to be the pullback of the square
\[ \xymatrix{ \mathcal{C}_2 \ar[d] \ar[r] &   \mathcal{D}(\Tilde{R}) \ar[d] \\ 
\operatorname{Fun}(\Delta^{1}, \mathcal{D}(\Tilde{R})) \ar[r] & \operatorname{Fun}(\Delta^{0}\sqcup \Delta^{0}, \mathcal{D}(\Tilde{R})),}\]
where the arrow in the bottom is the forgetful functor sending $(M\xrightarrow[]{f} N)$ to $(M,N)$ for $M, N\in \mathcal{D}(\Tilde{R})$ and the right vertical map sends $K \in  \mathcal{D}(\Tilde{R})$ to $(K, K)$.

The fact that the induced $\psi$-linear morphism $\gamma_{c_{\psi_{}}}: \rho^{*}(\mathscr{E}) \otimes_{\Tilde{R},\psi} S \rightarrow \rho^{*}(\mathscr{E})\otimes_{\Tilde{R}} S$ is the identity after modulo $\epsilon$ precisely means that after modulo $\epsilon$, $(\rho^{*}(\mathscr{E}),\gamma_{c_{\psi_{}}})$ (viewed as an object in $\mathcal{C}_1$) actually lies in $\mathcal{D}(\qd(\Tilde{R}))$, defined as follows.
\end{remark}
 

%Motivated by the above discussion, we make the following definition:
\begin{definition}\label{def. Rel MIC}
    Define $\mathcal{D}(\qd(\Tilde{R}))$ to be the pullback of the following diagram
\[ \xymatrix{ \mathcal{D}(\qd(\Tilde{R})) \ar[r] \ar[d] & \mathcal{C}_1 \ar[d] \\ 
\mathcal{D}(\Tilde{R}) \ar[r] &  \mathcal{C}_2  .}\]
and we will name this category as the \textit{derived category of $q$-connections over $\Tilde{R}$}. Here the right vertical map is given by modulo $\epsilon$ and the bottom arrow sends $M\in \mathcal{D}(\Tilde{R})$ to $(M\xrightarrow[]{\Id} M)$.

Similarly, we define $\Perf(\qd(\Tilde{R})$ (resp. $\Vect(\qd(\Tilde{R}))$) by replacing $\mathcal{D}(\bullet)$ with $\Perf(\bullet)$ (resp. $\Vect(\bullet)$) ((including such a modification for $\mathcal{C}_1$ and $\mathcal{C}_2$) in the above diagram. For $n\in \mathbb{N}$, by replacing $\mathcal{D}(\Tilde{R})$ with $\mathcal{D}(\Tilde{R}/d^n)$, we construct corresponding categories $\mathcal{D}(\qd(\Tilde{R}/d^n))$.
\end{definition}


As the geometry of stacks dominates the description of quasi-coherent complexes on it. Actually, in \cite{bhatt2022absolute} and \cite{bhatt2022prismatization}, which turns out to be  S  When translating 


leading to the classification studied the Hodge-Tate crystals over $\mathcal{O}_K$ in \cite{anschutz2022v} via a stacky approach. Actually, as the category of Hodge-Tate crystals on $(\mathcal{O}_K)_{\Prism}$ is equivalent to the category of vector bundles on the Hodge-Tate stack $\Spf(\mathcal{O}_K)^{\HT}$, it suffices to study the later. Under such a stacky perspective, the unramified case (i.e. $\mathcal{O}_K=W(k)$) was already treated in \cite{bhatt2022absolute}, while the general description was obtained in \cite{anschutz2022v}. More notably, such a stacky approach naturally leads to results for non-abelian coefficients, In particular, \cite{anschutz2022v} obtained a non-abelian version of \cite{gao2023hodge}.

%  (the advantage of such a stacky method will be illustrated in ) . 


We consider $Y=\Spf(R/(\Bar{x}_1,\cdots,\Bar{x}_r)) \hookrightarrow X$ to be a closed embedding with $(\Bar{x}_1,\cdots,\Bar{x}_r)$ a $p$-completely regular sequence relative to $\Bar{A}$ in the sense of \cite[Definition 2.42]{bhatt2022prisms}. We then fix a lift of this sequence in $\Tilde{R}$, which will be denoted as $(x_1,\cdots,x_r)$. Notice that such a lift of sequence forms a $(p,I)$-completely regular sequence relative to $A$. Write $J=(d,x_1,\cdots,x_r)\subseteq \Tilde{R}$. Under such assumptions \cite[Proposition 3.13]{bhatt2022prisms} then guarantees the existence of prismatic envelope with respect to the morphism of $\delta$-pairs $(\Tilde{R}, (d))\to (\Tilde{R}, J)$, which is given by $C=\Tilde{R}\{\frac{J}{d}\}^{\wedge}_{\delta}=\Tilde{R}\{\frac{x_1,\cdots,x_r}{d}\}^{\wedge}_{\delta}$.

 $\gamma_{b,c}$ gives a $\psi$-linear endomorphism on $\rho^{*}(\mathscr{E})[\epsilon]/\epsilon^2 \in \mathcal{D}(R)$, hence $(\rho^{*}(\mathscr{E}),\gamma_{b,c})$ lies in the category $\mathcal{C}_1$ defined to be the pullback of the following square:
    \[ \xymatrix{ \mathcal{C}_1 \ar[d] \ar[r] &   \mathcal{D}(A) \ar[d] \\ 
\operatorname{Fun}(\Delta^{1}, \mathcal{D}(R)) \ar[r] & \operatorname{Fun}(\Delta^{0}\sqcup \Delta^{0}, \mathcal{D}(R)) }.\]
Here the arrow in the bottom is the forgetful functor sending $(M\xrightarrow[]{f} N)$ to $(M,N)$ for $M, N\in \mathcal{D}(R)$ and the right vertical map sends $K \in  \mathcal{D}(A)$ to $(\psi^{*}K, K\otimes_A R)$.

Similarly, one could define the category $\mathcal{C}_2$ to be the pullback of the square
\[ \xymatrix{ \mathcal{C}_2 \ar[d] \ar[r] &   \mathcal{D}(A) \ar[d] \\ 
\operatorname{Fun}(\Delta^{1}, \mathcal{D}(A)) \ar[r] & \operatorname{Fun}(\Delta^{0}\sqcup \Delta^{0}, \mathcal{D}(A)),}\]
where the arrow in the bottom is the forgetful functor sending $(M\xrightarrow[]{f} N)$ to $(M,N)$ for $M, N\in \mathcal{D}(A)$ and the right vertical map sends $K \in  \mathcal{D}(A)$ to $(K, K)$.

The fact that the induced $\psi$-linear morphism $\gamma_{b,c}: \rho^{*}(\mathscr{E})\rightarrow \rho^{*}(\mathscr{E})\otimes_A R)$ is the identity after modulo $\epsilon$ precisely means that after modulo $\epsilon$, $(\rho^{*}(\mathscr{E}),\gamma_{b,c})$ (viewed as an object in $\mathcal{C}_1$) actually lies in $\mathcal{D}(\qd(A))$, defined as follows. 
\end{remark}


%Motivated by the above discussion, we make the following definition:
%\begin{definition}\label{def.MIC}Define $\mathcal{D}(\qd(A))$ to be the pullback of the following diagram\[ \xymatrix{ \mathcal{D}(\qd(A)) \ar[r] \ar[d] & \mathcal{C}_1 \ar[d] \\ \mathcal{D}(A) \ar[r] &  \mathcal{C}_2  .}\]and we will name this category as the \textit{derived category of $q$-connections over $A$}. Here the right vertical map is given by modulo $\epsilon$ and the bottom arrow sends $M\in \mathcal{D}(A)$ to $(M\xrightarrow[]{\Id} M)$. 

More concretely, an object in $\mathcal{D}(\qd(A))$ is given by a pair $(M,\gamma_M=\Id+\epsilon \partial_M)$ such that:
\begin{itemize}
    \item $M\in \mathcal{D}(A)$,
    \item $\gamma_M: M\otimes_{\Tilde{R},\psi} S\xrightarrow{\simeq} M\otimes_{A} R$
        given by the $R$-linear extension of $\gamma_M=\Id+\epsilon \partial_M$ on $M$ is an isomorphism, where $\psi: \to R$ is the $W(k)$-linear morphism defined in \cref{lemt.extend delta}.
\end{itemize}
The morphisms between two objects $(M,\gamma_M)$ and $(N,\gamma_N)$ in $\mathcal{D}(\qd(A))$ are given by\footnote{Strictly speaking, one can check that for $f\in \Hom_{\mathcal{D}(A)}(M,N)$,  $\partial_N\circ f-f\circ \partial_M\in \Hom_{\mathcal{D}(A}(M,\gamma_{0,*}N)$, i.e. $(\partial_N\circ f-f\circ \partial_M)(ax)=\gamma_0(a)(\partial_N\circ f-f\circ \partial_M)(x)$ for $a\in A$, but since $\Hom_{\mathcal{D}(A)}(M,N)$ and $\Hom_{\mathcal{D}(A}(M,\gamma_{0,*}N)$ have the same underlying complex (viewed as objects in $\mathcal{D}(W(k))$), we don't distinguish them here.} $$\Hom_{\mathcal{D}(\qd(A))}((M,\gamma_M), (N,\gamma_N))=\fib(\Hom_{\mathcal{D}(A)}(M,N)\xrightarrow{f\mapsto \partial_N\circ f-f\circ \partial_M} \Hom_{\mathcal{D}(A)}(M,N)).$$
Similarly, we define $\Perf(\qd(A)$ (resp. $\Vect(\qd(A))$) by replacing $\mathcal{D}(\bullet)$ with $\Perf(\bullet)$ (resp. $\Vect(\bullet)$) ((including such a modification for $\mathcal{C}_1$ and $\mathcal{C}_2$) in the above diagram. For $n\in \mathbb{N}$, by replacing $\mathcal{D}(A)$ with $\mathcal{D}(A/d^n)$, we construct corresponding categories $\mathcal{D}(\qd(A/d^n))$.
\end{definition}


\begin{remark}\label{rem.explicit description via sen operator}
    More explicitly, following the discussion before \cref{rem.describe the category}, we see that specifying an object in $\mathcal{D}(\qd(A))$ is the same as giving a pair $(M,\partial_M)$ where $M \in \mathcal{D}(A)$ and $\partial_M$ is an operator on $M$ satisfying a specific (twisted) Leibniz rule given in the following lemma. Actually, then $\gamma_M: \psi^{*}M=M\otimes_{A,\psi} R\to M\otimes_A R$ is the unique $R$-linear extension of $\Id+\epsilon \partial_M: M\to M\otimes_A R$.
\end{remark}


\begin{theorem}\label{thmt.old main classification}
Assume that $p>2$ or $\alpha>0$. Let $n\in \mathbb{N}\cup \{\infty\}$. The functor 
    \begin{align*}
        &\beta_n^{+}: \mathcal{D}(X_n^{\Prism}) \rightarrow \mathcal{D}(A/d^n[\partial; \gamma_A, \partial_A]), \qquad \mathcal{E}\mapsto (\rho^{*}(\mathcal{E}),\partial_{\mathcal{E}})
        %\\ resp. ~&\beta_n^{+}: \mathcal{D}(X^{\Prism}_n) \rightarrow \mathcal{D}(\qd(A/d^n)), \qquad \mathcal{E}\mapsto (\rho^{*}(\mathcal{E}),\partial_{\mathcal{E}})
    \end{align*}
    constructed in \cref{prop. induce functor} is fully faithful. %\footnote{Here $\mathcal{D}(\mathrm{MIC}(\mathfrak{S}[[\frac{E}{p}]])$ is defined similarly as \cref{def.MIC}}. 
     Moreover, its essential image consists of those objects $M\in \mathcal{D}(A/d^n[\partial; \gamma_A, \partial_A])$ %(resp. $M\in \mathcal{D}(\qd(A/d^n))$) 
     satisfying the following pair of conditions:
    \begin{itemize}
        \item $M$ is $(p,d)$-complete.
        \item The action of $\partial_M$ on the cohomology $\mathrm{H}^*(M\otimes^{\mathbb{L}}k)$ \footnote{Here the derived tensor product means the derived base change along $A/d^n\to A/(d,q-1)=k$.} is locally nilpotent. 
    \end{itemize}
\end{theorem}
\begin{proof}%[Proof of \cref{thmt.main classification}]
The functor is well-defined thanks to \cref{prop. induce functor}. Then we follow the proof of \cite[Theorem 3.5.8]{bhatt2022absolute}. 
    For the full faithfulness, let $\mathcal{E}$ and $\mathcal{F}$ be quasi-coherent complexes on $X^\Prism_n$ and we want to show that the natural map 
    \begin{equation*}
        \Hom_{\mathcal{D}(X^\Prism_n)}(\mathcal{E}, \mathcal{F}) \rightarrow \Hom_{\mathcal{D}(A/d^n[\partial; \gamma_A, \partial_A])} (\rho^{*}(\mathcal{E}), \rho^{*}(\mathcal{F}))
    \end{equation*}
    is a homotopy equivalence. Thanks to \cref{propt.generation}, we could reduce to the case that $\mathcal{E}=\mathcal{I}^k$ for some $k\in \mathbb{Z}$. Replacing $\mathcal{F}$ by the twist $\mathcal{F}(-k)$, we could further assume that $k=0$. Then the desired result follows from \cref{propt. sen calculate cohomology} and \cref{rem. cohomology of the structure sheaf}. 
    
    
\end{proof}
%\begin{proposition}
%There is an equivalence of categories $$\mathcal{D}(\TWCart_{[n]}) \rightarrow \lim _{(A, I)} \widehat{\mathcal{D}}(A/I^{p^n}[\frac{I^p}{p}])$$ Here $A/I^{p^n}[\frac{I^p}{p}]$ denote the sub-$A/I^{p^n}$ algebra generated by $1$ and $\frac{I^p}{p}$ inside $A/I^{p^n}[\frac{1}{p}]$.
%\end{proposition}

\begin{corollary}\label{corot.perfect version of the remain theorem}
Let $n\in \mathbb{N}\cup \{\infty\}$.. The functor $\beta^+_n$ from \cref{thmt.main classification} restricts to a fully faithful functor
  \[
    \beta^+_n\colon \Perf(X_n^{\Prism}) \to \Perf(\qd(A/d^n))%\footnote{Here $\Perf(\mathrm{MIC}(\mathfrak{S}[[\frac{E}{p}]]/(\frac{E}{p})^n)$ is defined to be the $\infty$-category of perfect complexes $M$ over $\mathfrak{S}[[\frac{E}{p}]]/(\frac{E}{p})^n$ admitting a $W(k)$-linear operator $\Theta$ from $M$ to itself satisfying the Leibniz rule. In particular, when $n=1$, as $\Theta$ vanishes on the $\mathfrak{S}/E$, this coincides with $\Perf(\mathcal{O}_K[\Theta_{\pi}])$  defined in \cite{anschutz2022v} by the proof of \cite[Lemma 2.13]{anschutz2022v}.}
  \]
  whose essential image consists of $p$-adically complete perfect complexes $M$ over $A/d^n$ admitting a $W(k)$-linear operator $\partial$ from $M$ to itself satisfying the Leibniz rule such that $\partial^p-(d^{\prime}(q))^{p-1}\Theta$ is nilpotent on $H^\ast(k\otimes^L M)$.    
\end{corollary}
\begin{proof}
    This follows from our definition of $\Perf(\qd(A/d^n))$ given in \cref{def.MIC} and \cref{thmt.main classification} directly.
\end{proof}
\begin{remark}\label{rem.describe the category}
We consider the $1$-truncated simplicial scheme 
\[\begin{tikzcd}
    T_{\bullet}=(\Spf(R)\arrow[r, altstackar=3] & \Spf(A))
\end{tikzcd}\]
and let $\mathscr{T}:=\colim T_{\bullet}$ be the associated stack. Here $d_{0}^1=\psi: \Spf(R)\to \Spf(A)$ is introduced in \cref{lemt.extend delta}, $d_{1}^1=\iota: \Spf(R)\to \Spf(A)$ corresponds to the canonical inclusion, and $s_0^0: \Spf(A)\to \Spf(R)$ is the morphism given by modulo $\epsilon$. Let $\Mod_{\mathscr{T}}=\mathcal{D}(\mathscr{T})^{\heartsuit}$ be the heart of quasi-coherent complexes on $\mathscr{T}$, then $\mathcal{D}(\mathscr{T})=\mathcal{D}(\Mod_{\mathscr{T}})$ as $T_{\bullet}$ is a finite diagram with affine terms. On the other hand, notice that 
\[\begin{tikzcd}
    \Mod_{\mathscr{T}}=\Tot(\Mod_A\arrow[r, altstackar=3] & \Mod_R)
\end{tikzcd},\]
hence specifying an object $\mathcal{M}$ in $\Mod_{\mathscr{T}}$ leads to a pair $(M,\gamma_M)$ such that $M$ is an $A$-module,  $\gamma_M: M\otimes_{A,\psi} R \stackrel{\simeq}{\longrightarrow} M\otimes_{A,\iota} R$ is a $R$-linear isomorphism which reduces to the identity after modulo $\epsilon$. For our purpose, it will be more convenient to work with a derivation $\partial_M$ on $M$ instead, see the following lemma.
\end{remark}
\begin{lemma}\label{lem.leibniz}
   Given a pair $(M,\gamma_M)$ as above, we can write $\gamma_M$ as $\Id+\epsilon \partial_M$ when restricted to $M$ for a functor $\partial_M: M\to M$, then we have that $$\partial_M(ax)=a\partial_M(x)+\partial(a)x+q(q^{p^\alpha}-1) \partial(a)\partial_M(x)$$ for $a\in A$ and $x\in M$, here $\partial: A\to A$ is $W(k)$-linear and sends $q^i$ to $[pi]_{q^{p^\alpha}} q^{i-1}$. In particular, 
   $$\partial_M(qx)=[p]_{q^{p^\alpha}}x+q^{p^{\alpha+1}+1}\partial_M(x).$$
\end{lemma}
\begin{proof}
    The characterization of $\partial$ on $A$ follows as $\gamma$ is $\psi$-linear and $\psi (q^i)=q^i+\epsilon [pi]_{q^{p^\alpha}} q^{i-1}$. For a general pair $(M,\gamma_M)$,
    \begin{equation*}
        \begin{split}
            &\gamma_M(ax)=\psi(a)\gamma_M(x)=(a+\epsilon\partial(a))(x+\epsilon\partial_M(x))\\=&ax+\epsilon(a\partial_M(x)+\partial(a)x)+\epsilon^2 \partial(a)\partial_M(x)\\=&ax+\epsilon(a\partial_M(x)+\partial(a)x)+\epsilon q(q^{p^\alpha}-1) \partial(a)\partial_M(x)
            \\=&ax+\epsilon(a\partial_M(x)+\partial(a)x+q(q^{p^\alpha}-1) \partial(a)\partial_M(x)).
        \end{split}
    \end{equation*}
    This implies the desired result.
\end{proof}
\begin{remark}
    $\partial_M$ preserves the $d$-adic filtration, i.e. $\partial(dM)\subseteq dM$ as $\partial(d)\in d A$.
\end{remark}

Motivated by \cref{lem.leibniz}, the following skew polynomial enters the picture.
\begin{definition}\label{def.skew polynomial}
    Let $\gamma_A: A\to A$ be the ring automorphism, then $\partial_A: A\to A$ is a $\gamma_A$-derivation of $A$, i.e. $\partial_A(x_1x_2)=\gamma_A(x_1)\partial_A(x_2)+\partial_A(x_1)x_2$, then we define the \textit{Ore extension} $A[\partial; \gamma_A, \partial_A]$ to be the noncommutative ring obtained by giving the ring of polynomials $A[\partial]$ a new multiplication, subject to the identity
    $$\partial r=\gamma_A(r)\partial+\partial_A(r), ~~~\forall r\in A.$$
\end{definition}
\begin{remark}\label{rem. mod d ore extension}
    For any $n\geq 1$, as $\gamma_A$ (resp. $\partial_A$) induces a ring automorphism $A/d^n \to A/d^n$ (resp. a $\gamma_A$-derivation of $A/d^n$), we can similarly define $A/d^n[\partial; \gamma_A, \partial_A]$. Note that one $n=1$, $A/d[\partial; \gamma_A, \partial_A]$ is just the usual (commutative) polynomial ring $A/d[\partial]$ as $\gamma_A$ reduces to the identity after modulo $d$ and $\partial_A$ vanishes on $A/d$.
\end{remark}
\begin{remark}\label{rem. cohomology of the structure sheaf}
   One can check that $A$ is isomorphic to the quotient of $A[\partial; \gamma_A, \partial_A]$ by the left ideal $(\partial)$. More precisely, there is a canonical resolution for $A$ by finite free $A[\partial; \gamma_A, \partial_A]$-modules:
   $$[A[\partial; \gamma_A, \partial_A] \stackrel{\times \partial}{\longrightarrow} A[\partial; \gamma_A, \partial_A]]\simeq A.$$
   Consequently, for $M\in \mathcal{D}(A[\partial; \gamma_A, \partial_A])$, 
   $$\RHom_{\mathcal{D}(A[\partial; \gamma_A, \partial_A])}(A, M)=[M\stackrel{ \partial}{\longrightarrow} M].$$
   Such an observation will be used to calculate the cohomology later.
\end{remark}

Combining \cref{lem.leibniz} with the discussion above it, we obtain a functor 
\begin{equation*}
  \begin{split}
      \Mod_{\mathscr{T}} &\to \Mod_{A[\partial; \gamma_A, \partial_A]}\\
      \mathcal{E} &\mapsto (\rho^{*}\mathcal{E}, \partial_{\mathcal{E}})
  \end{split}
  \end{equation*}


   

The above discussion can be summarized as follows:
\begin{proposition}\label{prop. induce functor}
  For $n\in \mathbb{N}\cup \{\infty\}$, the pullback along $\rho: \Spf(A/d^n)\to X_n^{\Prism}$ induces a functor 
  \begin{equation*}
  \begin{split}
      \mathcal{D}(X_n^{\Prism}) &\to \mathcal{D}(A/d^n[\partial; \gamma_A, \partial_A])\\
      \mathcal{E} &\mapsto (\rho^{*}\mathcal{E}, \partial_{\mathcal{E}})
  \end{split}
  \end{equation*}
  which will be denoted as $\beta_n^+$ later. Here $\partial_{\mathcal{E}}$ is defined after \cref{cort.truncated}.
\end{proposition}





\begin{remark}\label{rem. compatibility with GSQ}
    When $\alpha=0$, $\partial_M$ satisfies the same Leibniz rule defining $q(p)$-connection in \cite{gros2023absolute}, hence in this case
    $\Vect(\qd(A))$ coincides with the category of finite projective $A$ modules equipped with a $q(p)$-connection studied in \textit{loc.cit.}, denoted as $\nabla_{q(p)} (A)$ there.
\end{remark}

 In other words, we need to show that for every nonzero object $M\in \mathcal{C}$, $M$ admits a nonzero morphism from $\rho^*(\mathcal{I})^k[m]$ for some $m,k \in \mathbb{Z}$. Replacing $M$ by $M\otimes k$ (the noncommutative derived Nakayama guarantees that $L\otimes k$ detects whether $L$ is zero or not for $(p,d)$-complete $M$), we may assume that there exists some cohomology group $\mathrm{H}^{-m}(M)$ containing a nonzero element killed by $\partial$ (this could be done by iterating the action of $\partial$ and then use the nilpotence assumption). %Furthermore, we could assume this element is actually killed by $\partial-ke$ for a single integer $k$. 
    It then follows that there exists a non-zero morphism from $\rho^*(\mathcal{O})[m]$ to $M$.

Motivated by \cref{prop. rel two derivation vanish} and the discussion above it, following the roadmap leading to \cref{def.MIC}, we end up with the following category in which $(\rho^*\mathcal{E}, \nabla_{\mathcal{E}}=\sum_{i=1}^m \nabla_{\mathcal{E},i}\otimes dT_i)$ lives.
\begin{definition}\label{def. Rel q higgs}
We define $\mathcal{D}(\qh(\Tilde{R}))$ as follows and will name this category as the \textit{derived category of $q$-Higgs derivations over $\Tilde{R}$}. An object in $\mathcal{D}(\qh(\Tilde{R}))$ is given by a pair $(M, \gamma_M=\Id+\epsilon \nabla_M)$ such that the following holds:
    \begin{itemize}
        \item $M\in \mathcal{D}(\Tilde{R})$.
        \item $\gamma_M: M\otimes_{\Tilde{R},\psi} S\xrightarrow{\simeq} M\otimes_{\Tilde{R}} S$
        given by the $S$-linear extension of $\gamma_M=\Id+\epsilon \nabla_M$ on $M$ is an isomorphism, where $\psi$ is the $A$-linear morphism defined in \cref{lem. twist S in the relative case}.
        \item $\nabla_M \wedge \nabla_M=0$, i.e. if $\nabla_M =\sum_{i=1}^m \nabla_{M,i}\otimes dT_i$, then $\nabla_{M,i}\circ \nabla_{M,j}=\nabla_{M,j}\circ \nabla_{M,i}$.
    \end{itemize}
 The morphisms between two objects $(M,\gamma_M)$ and $(N,\gamma_N)$ in $\mathcal{D}(\qh(\Tilde{R}))$ are given by the de Rham complex of $\Hom_{\mathcal{D}(\Tilde{R})}(M,N)$. More precisely, let $P=\Hom_{\mathcal{D}(\Tilde{R})}(M,N)$, we can define operators $\nabla_{P,i}: P\to 
 P$ such that $\nabla_{P,i}(f)=\nabla_{N,i}\circ f-f\circ \nabla_{M,i}$\footnote{Strictly speaking, one can check that for $f\in P$,  $\nabla_{P,i}(f)\in \Hom_{\mathcal{D}(\Tilde{R})}(M,\gamma_{i,*}N)$, i.e. $\nabla_{P,i}(f)(ax)=\gamma_i(a)\nabla_{P,i}(f)(x)$ for $a\in \Tilde{R}$, but since $P$ and $\Hom_{\mathcal{D}(\Tilde{R})}(M,\gamma_{i,*}N)$ have the same underlying complex (viewed as objects in $\mathcal{D}(A)$), we don't distinguish them here.},  then 
 \begin{equation*}
 \begin{split}
     &\Hom_{\mathcal{D}(\qh(\Tilde{R}))}((M,\gamma_M), (N,\gamma_N))
     \\=&(P\xrightarrow{\nabla_P} P\otimes_{\Tilde{R}} \Omega_{\Tilde{R}/A}\xrightarrow{\nabla_{P}\wedge \nabla_{P}} \cdots \to P\otimes_{\Tilde{R}} \Omega_{\Tilde{R}/A}^{m}\to 
        0),
\end{split}
\end{equation*}
where $\nabla_{P}=\sum_{i=1}^m \nabla_{P,i}\otimes dT_i$. Later we will call the complex above the \textit{de Rham complex of $(P,\nabla_P)$} and denote it as $\mathrm{DR}(P,\nabla_P)$.

Similarly, one defines $\mathcal{D}(\qh(\Tilde{R}/d^n))$ for all $n$.
\end{definition}


\begin{remark}
    Concretely, an object in $\mathcal{D}(\qh(\Tilde{R}))$ is given by a pair $(M, \gamma_M)$ such that $M\in\mathcal{D}(\Tilde{R})$ and $\gamma_M$ is a $S$-linear morphism $M\otimes_{\Tilde{R},\psi} S\to M\otimes_{\Tilde{R}} S$ which reduces to the identity map after modulo $\epsilon$. The later condition then forces $\gamma_M: M\otimes_{\Tilde{R},\psi} S\to M\otimes_{\Tilde{R}} S$ to be an isomorphism. This essentially follows from the fact that $1+\epsilon dT_i\in S$ has an inverse, given by $1-\frac{1}{1+\beta T_i}\cdot\epsilon dT_i \in S$ (here the notation makes sense as $\beta=q-1$ and $\Tilde{R}$ is $(q-1)$-adically complete)).
\end{remark}

\begin{remark}[$\gamma_M$ leads to the twisted Leibnitz rule]\label{rem. relative explicit description via sen operator}
    More explicitly, following the discussion before \cref{prop. rel two derivation vanish}, we see that to specify an object in $\mathcal{D}(\qh(\Tilde{R}))$, it suffices to give a pair $(M,\nabla_M=\sum_{i=1}^m \nabla_{M,i}\otimes dT_i)$ with $M \in \mathcal{D}(\Tilde{R})$ and $\nabla_{M,i}: M\to M$ commuting operators on $M$ satisfying specific (twisted) Leibniz rules given in the following lemma. Actually, then $\gamma_M: \psi^{*}M=M\otimes_{\Tilde{R},\psi} S\to M\otimes_A S$ is the unique $S$-linear extension of $\Id+\epsilon \nabla_M: M\to M\otimes_{\Tilde{R}} S$.
\end{remark}

\begin{remark}
    We point out that when $(M,\gamma_M)=(\Tilde{R}, \psi)$, then $$\Hom_{\mathcal{D}(\qh(\Tilde{R}))}((M,\gamma_M), -)$$ can be calculated via the de Rham complex of $N$, which will be useful later. Indeed, if writing $\gamma_N$ as $\gamma_N=\Id+\epsilon\nabla_N=\Id+\epsilon\sum_{i=1}^m\nabla_{N,i}dT_i$, then after identifying $P=\Hom_{\mathcal{D}(\Tilde{R})}(\Tilde{R},N)$ with $N$ by evaluating $f\in P$ at $1$, one observes that 
    $\nabla_{P,i}$ becomes $\nabla_{N,i}$,
    hence 
    \begin{equation*}
    \begin{split}
        \Hom_{\mathcal{D}(\qh(\Tilde{R}))}((\Tilde{R},\psi), (N,\gamma_N))=(N\xrightarrow{\nabla_N} N\otimes_{\Tilde{R}} \Omega_{\Tilde{R}/A}\xrightarrow{\nabla_{N}\wedge \nabla_{N}} \cdots \to N\otimes_{\Tilde{R}} \Omega_{\Tilde{R}/A}^{m}\to 
        0)
    \end{split}
    \end{equation*}
    is exactly given by $\mathrm{DR}(N,\nabla_N)$.
\end{remark}
\begin{remark}%[Cohomology of a $q$-Higgs derivation]




   Indeed, 
   
   Consequently, for $N$ an object in, , we have that
   $$[N\xrightarrow{\nabla_N:=\sum \nabla_i\otimes dT_i} N\otimes_{\Tilde{R}} \Omega_{\Tilde{R}/A}\xrightarrow{\nabla_{N}\wedge \nabla_{N}} \cdots \to N\otimes_{\Tilde{R}} \Omega_{\Tilde{R}/A}^{m}\to 
        0].$$
   We will call the right-hand side of the above equation the \textit{$q$-de Rham complex of $N$}, denoted as $\mathrm{DR}(N)$. Such an observation will be used to calculate the cohomology later.
\end{remark}

\begin{definition}\label{def. enhanced q higgs}
   We define $\mathcal{D}(\qe(\Tilde{R}))$ as follows and will name it as the category of \textit{enhanced $q$-Higgs modules} over $\Tilde{R}$. An object in $\mathcal{D}(\qe(\Tilde{R}))$ is given by a pair $(M, \gamma_M=\Id+\epsilon_0\partial_M+\epsilon \nabla_M)$ such that the following holds:
    \begin{itemize}
        \item $M\in \mathcal{D}(\Tilde{R})$,
        \item $\gamma_M: M\otimes_{\Tilde{R},\psi} S\xrightarrow{\simeq} M\otimes_{\Tilde{R}} S$
        given by the $S$-linear extension of $\gamma_M=\Id+\epsilon_0\partial_M+\epsilon \nabla_M$ on $M$ is an isomorphism, where $\psi$ is defined in \cref{lem. AR twist S in the relative case}.
        \item $\nabla_M \wedge \nabla_M=0$, i.e. if writing $\nabla_M$ as $\sum_{i=1}^m \nabla_{M,i}\otimes dT_i$, then $\nabla_{M,i}\circ \nabla_{M,j}=\nabla_{M,j}\circ \nabla_{M,i}$.
        \item $\nabla_{M,i}$ and $\partial_{M}$ satisfies the relation stated in \cref{lem. AR relation between 0 and i}, i.e. 
        \begin{equation*}
    \nabla_{M,i}(1-\beta q \mathscr{D}(\nabla_{M,i}))\circ \partial_M=s_0(\partial_M-s_0^{-1}\mathscr{D}(\nabla_{M,i})+s_1)\circ \nabla_{M,i},
\end{equation*}
    \end{itemize}
Let $P=\Hom_{\mathcal{D}(\Tilde{R})}(M,N)$. The morphisms between objects $(M, \gamma_M)$ and $(N, \gamma_N)$ are given by the total complex of $$[\mathrm{DR}(P,\nabla_P)\xrightarrow{\partial_P^{[\bullet]}} \mathrm{DR}(P,\nabla_P)],$$ 
where $\mathrm{DR}(P,\nabla_P)$ is introduced in \cref{def. Rel q higgs} and the induced map $\partial_P^{[\bullet]}$ is defined in \cref{propt. AR factor through fiber}.

Similarly, one defines $\mathcal{D}(\qe(\Tilde{R}/d^n))$ for all $n$.
\end{definition}

Then following the discussion between \cref{prop. rel two derivation vanish} and \cref{prop. relative induce functor} by taking \cref{propt.key automorphism of functors AR} (resp. \cref{prop. AR two derivation vanish}) as the input replacing \cref{propt.key automorphism of functors relative case} (resp. \cref{prop. rel two derivation vanish}), we end up with the following category in which $(\rho_X^*\mathcal{E}, \partial_{\mathcal{E}}, \nabla_{\mathcal{E}}=\sum_{i=1}^m \nabla_{\mathcal{E},i}\otimes dT_i)$ lives.

Following the discussion above \cref{propt. relative factor through fiber}, we conclude that
\begin{proposition}\label{propt. AR factor through fiber}
    For $n\in \mathbb{N}\cup \{\infty\}$ and $\mathcal{E}\in \mathcal{D}(X_{ n}^{\Prism})$, the natural morphism $\mathrm{R} \Gamma(X_{n}^{\Prism}, \mathcal{E})\to \rho_X^{*}\mathcal{E}$ induces a canonical morphism $$
    \mathrm{R} \Gamma(X_{n}^{\Prism}, \mathcal{E})\to \fib(\rho_X^*\mathcal{E}\stackrel{\nabla_{\mathcal{E},i}}{\longrightarrow} \rho_X^*\mathcal{E}).$$
    for all $i$ (here we abuse the notation by viewing $\nabla_{\mathcal{E},0}$ as $\partial_{\mathcal{E}}$). Hence it induces a canonical morphism
    \begin{equation*}
        \mathrm{R} \Gamma(X_{n}^{\Prism}, \mathcal{E})\to \fib(\mathrm{DR}(\rho_X^*\mathcal{E},\nabla_{\mathcal{E}})\xrightarrow{\partial_{\mathcal{E}}^{[\bullet]}} \mathrm{DR}(\rho_X^*\mathcal{E},\nabla_{\mathcal{E}})),
    \end{equation*}
    where the later is defined as the total complex of
    \[\xymatrixcolsep{2pc}\xymatrix{\rho_X^*\mathcal{E}\ar[d]^{\partial_{\mathcal{E}}}\ar[r]^-{\nabla_{\mathcal{E}}}& \rho_X^*\mathcal{E}\otimes_{\Tilde{R}/I^n} \Omega^1_{(\Tilde{R}/I^n)/(A/I^n)} \ar[d]_{}^{\partial^{[1]}_{\mathcal{E}}}\ar[r] &\cdots \ar[d]\ar[r] & \rho_X^*\mathcal{E}\otimes_{\Tilde{R}/I^n} \Omega^m_{(\Tilde{R}/I^n)/(A/I^n)} \ar[d]^{\partial^{[m]}_{\mathcal{E}}}\ar[r] &0
\\ \rho_X^*\mathcal{E}\ar[r]^-{\nabla_{\mathcal{E}}}& \rho_X^*\mathcal{E}\otimes_{\Tilde{R}/I^n} \Omega^1_{(\Tilde{R}/I^n)/(A/I^n)}\ar[r]& \cdots \ar[r] & \rho_X^*\mathcal{E}\otimes_{\Tilde{R}/I^n} \Omega^m_{(\Tilde{R}/I^n)/(A/I^n)} \ar[r] &0,}\]
here $\partial^{[t]}_{\mathcal{E}}:=a_t(\nabla_{\mathcal{E}}) \partial_{\mathcal{E}}+b_t(\nabla_{\mathcal{E}})$ with $a_1(\nabla_{\mathcal{E}})=s_0(1-\beta q\mathscr{D}(\nabla_{\mathcal{E}}))^{-1},~ b_1(\nabla_{\mathcal{E}})=(1-\beta q\mathscr{D}(\nabla_{\mathcal{E}}))^{-1}(s_1-\mathscr{D}(\nabla_{\mathcal{E}}))$ and $a_t, b_t$ defined inductively via 
\begin{equation*}
    a_{i+1}(\nabla_{\mathcal{E}})=a_{i}(\nabla_{\mathcal{E}})a_1(\nabla_{\mathcal{E}}),\quad b_{i+1}(\nabla_{\mathcal{E}})=a_{i}(\nabla_{\mathcal{E}})b_1(\nabla_{\mathcal{E}})+b_i(\nabla_{\mathcal{E}}).
\end{equation*}
\end{proposition}
\begin{proof}
The proof of \cref{propt. relative factor through fiber} still works here. We just need to notice that $\partial_{\mathcal{E}}$ and $ \nabla_{\mathcal{E}}$ satisfies the last condition in \cref{def. enhanced q higgs}, hence $\partial^{[t]}_{\mathcal{E}}$ defined in this way makes the complex commute:
\begin{equation*}
    \begin{split}
        \nabla_{\mathcal{E}}\circ \partial_{\mathcal{E}}^{[t]}&=\nabla_{\mathcal{E}}\circ (a_t(\nabla_{\mathcal{E}}) \partial_{\mathcal{E}}+b_t(\nabla_{\mathcal{E}}))
        \\&=a_t(\nabla_{\mathcal{E}}) ((a_1(\nabla_{\mathcal{E}})\circ \partial_{\mathcal{E}}+b_1(\nabla_{\mathcal{E}}))\circ \nabla_{\mathcal{E}})+b_t(\nabla_{\mathcal{E}})\circ\nabla_{\mathcal{E}} 
        \\&=(a_t(\nabla_{\mathcal{E}})a_1(\nabla_{\mathcal{E}})\circ \partial_{\mathcal{E}}+(a_t(\nabla_{\mathcal{E}})b_1(\nabla_{\mathcal{E}})+b_t(\nabla_{\mathcal{E}})))\circ\nabla_{\mathcal{E}}\\&=\partial_{\mathcal{E}}^{[t+1]}\circ\nabla_{\mathcal{E}}.
    \end{split}
\end{equation*}
Here we implicitly use the fact that both $a_t(\nabla_{\mathcal{E}})$ and $b_t(\nabla_{\mathcal{E}})$ commute with $\nabla_{\mathcal{E}}$. 
\end{proof}

More precisely, we can define the following category in which $(\rho_X^*\mathcal{E}, \partial_{\mathcal{E}}, \nabla_{\mathcal{E}}=\sum_{i=1}^m \nabla_{\mathcal{E},i}\otimes dT_i)$ lives.
\begin{definition}\label{def. ARL define the target category}
    We define $\mathcal{D}(\qe(\XY))$ as follows and will name it as the category of \textit{enhanced $q$-Higgs modules} over $\XY$. An object in $\mathcal{D}(\qe(\XY))$ is given by a pair $(M, \gamma_M=\Id+\epsilon_0\partial_M+\epsilon \nabla_M)$ such that the following holds:
    \begin{itemize}
        \item $M\in \mathcal{D}(\XY)$,
        \item $\gamma_M: M\otimes_{\XY,\psi} (\XY\otimes_{\Tilde{R}} S)\xrightarrow{\simeq} M\otimes_{\XY} (\XY\otimes_{\Tilde{R}} S)$
        given by the $\XY\otimes_{\Tilde{R}} S$-linear extension of $\gamma_M=\Id+\epsilon_0\partial_M+\epsilon \nabla_M$ on $M$ is an isomorphism, where $\psi$ is defined in \cref{lemt.ARL lci case appl extend eta}.
        \item $\nabla_M =\sum_{i=1}^m \nabla_{M,i}\otimes dT_i$ such that $\nabla_{M,i}\circ \nabla_{M,j}=\nabla_{M,j}\circ \nabla_{M,i}$.
        \item $\nabla_{M,i}$ and $\partial_{M}$ satisfies the relation stated in \cref{lem. AR relation between 0 and i}, i.e. 
        \begin{equation*}
    \nabla_{M,i}(1-\beta q \mathscr{D}(\nabla_{M,i}))\circ \partial_M=s_0(\partial_M-s_0^{-1}\mathscr{D}(\nabla_{M,i})+s_1)\circ \nabla_{M,i},
\end{equation*}
    \end{itemize}
The morphisms between objects $(M, \gamma_M)$ and $(N, \gamma_N)$ are similarly defined as that in \cref{def. enhanced q higgs}. 

Similarly, one defines $\mathcal{D}(\qe(\Tilde{R}/d^n))$ for all $n$.
\end{definition}


one can first show that $\mathcal{D}(C_{\infty})$ is generated under shifts and colimits by the invertible sheaves $\mathcal{I}^k$ for $k\in \mathbb{Z}$ reduce to the previous cases by noticing that 

our $q$-connection $\partial_{\mathcal{E}}$ on $\rho^{*}\mathcal{E}\in \mathcal{D}(\mathcal{O}_K)$ is different from the Sen operator on $\rho^{\prime *}\mathcal{E}$ for $\rho^{\prime}: \Spf(\mathcal{O}_K) \to X^{\HT}$ induced by the Breuil-Kisin prism associated to $X$ constructed in \cite{anschutz2022v}. Indeed, they differ by a unit. See \cref{example.action on generators} and \cite[Example 2.4]{anschutz2022v}. This reflects that various monodromy/Sen operators depend on the chart we chose and are not \textit{canonical}.

, which should be equivalent to our category $\Vect(\qh(\XY))$ modulo some technical issues

Specifying an object in $\mathcal{D}(\WCart)$ is the same as giving a pair $(M, \gamma_M=\Id+\epsilon\partial_M)\in \mathcal{D}(\qd(A))$ equipped with an action of $\mathbb{F}_p^{\times}$ such that\begin{itemize} 
\item $M\in \mathcal{D}(A)$ is $(p,d)$-complete. The $\mathbb{F}_p^{\times}$-action on $M\in \mathcal{D}(A)$ is semi-linear and commutes with $\gamma$, here the $\mathbb{F}_p^{\times}$-action on $A$ and $\epsilon$ is regulated in Section 3.4.
\item $M$ admits an $\mathbb{F}_p^{\times}$-invariant basis, i.e. $M=M^{\mathbb{F}_p^{\times}}\otimes_{A^{\mathbb{F}_p^{\times}}} A$.
\item After modulo $d$, taking $\mathbb{F}_p^{\times}$-invariants of $\gamma_M$ induces a monodromy operator $\partial_M^{\prime}: (M/d)^{\mathbb{F}_p^{\times}}\to (M/d)^{\mathbb{F}_p^{\times}}$ satisfying that the action of $(\partial_{M}^{\prime})^p-\partial_{M}^{\prime}$ on the cohomology $\mathrm{H}^*((M/d)^{\mathbb{F}_p^{\times}}\otimes_{\mathbb{Z}_p}^{\mathbb{L}}\mathbb{F}_p)$ is locally nilpotent. \footnote{In particular, the definition of $\partial_M^{\prime}$ implies that $\partial_M= \partial_M^{\prime}\otimes e$ after identifying $M/d$ with $(M/d)^{\mathbb{F}_p^{\times}}\otimes_{\mathbb{Z}_p} \mathcal{O}_K$.}\end{itemize}

Let us briefly explain the non-commutative ring shown up in this theorem.
%, cf. \cref{def.MIC} and \cref{rem.explicit description via sen operator} for full details. 
\begin{definition}[]\label{intro. definition of q connections}
   
\end{definition}
